Symbol Preference Aware Generative Models for Recovering Variable Names from Stripped Binary

Decompilation aims to recover the source code form of a binary executable. It has many security applications, such as malware analysis, vulnerability detection, and code hardening. A prominent challenge in decompilation is to recover variable names. We propose a novel technique that leverages the strengths of generative models while mitigating model biases. We build a prototype, GenNm, from pre-trained generative models CodeGemma-2B, CodeLlama-7B, and CodeLlama-34B. We finetune GenNm on decompiled functions and teach models to leverage contextual information. GenNm includes names from callers and callees while querying a function, providing rich contextual information within the model's input token limitation. We mitigate model biases by aligning the output distribution of models with symbol preferences of developers. Our results show that GenNm improves the state-of-the-art name recovery precision by 5.6-11.4 percentage points on two commonly used datasets and improves the state-of-the-art by 32% (from 17.3% to 22.8%) in the most challenging setup where ground-truth variable names are not seen in the training dataset.

==> rev-sum.tex <==


\setcounter{subsection}{0}
\setcounter{page}{1}

\onecolumn

{
\centering
\subsection*{\textbf{Revision Summary}}
}

We thank the reviewers for their detailed and constructive comments. In this document, we first summarize the changes we introduce during the revision in Section~\ref{sec:soc}. Then we elaborate how those changes address the revision requirements in Section~\ref{sec:rr}. After that, we discuss how we address other questions discussed in the reviews in Section~\ref{sec:other}.

\subsection{Summary of Changes}
\label{sec:soc}


Following the revision expectations in the review, we have substantially enhanced our submission in the following aspects: 
\begin{itemize}
    \item [\ref{sec:sub:clarify-contrib}] Clarify the contribution of \toolname compared to existing work. 
    \item [\ref{sec:sub:art-aval}] Clarify artifact availability.
    \item [\ref{sec:sub:exp-set}] Clarify experimental setups.
    \item [\ref{sec:sub:cmp-resym}] Add experiments to compare \toolname with ReSym.
    \item [\ref{sec:sub:cmp-split-by-func}] Add experiments to compare with baselines on the split-by-function setup.
    \item [\ref{sec:sub:more-ds}] Add experiments on more datasets with different optimization levels.
    \item [\ref{sec:sub:study-model-size}] Add experiments to show the effects of larger models.
    \item [\ref{sec:sub:bb-clm}] Add experiments to compare \toolname with programming-focused black-box LLMs.
    \item [\ref{sec:sub:general-rare-name}] Use experiments to justify how \toolname generalizes better to rare names.
    \item [\ref{sec:sub:abl-nv}] Add ablation study for the name validation algorithm.
    \item [\ref{sec:sub:abl-docs}] Add ablation study for the degree of context sensitivity.
    \item [\ref{sec:sub:sem-copy}] Validate assumptions about semantics consistency and variable copies.
    \item [\ref{sec:sub:mem-buf}] Validate the observation that the name {\tt memset} and {\tt buffer} are correlated.
    \item [\ref{sec:sub:long-ctx-code}] Clarify the challenges of reasoning long context code.
\end{itemize}

\subsubsection{\textbf{Clarify the contribution of \toolname compared to existing work}}
\label{sec:sub:clarify-contrib}
ReSym~\cite{resym} aims to recover names, types, and data structures. It shares a common goal with \toolname on name recovery. It fine-tunes an LLM for renaming variables and uses program analysis as a post-processing step. In particular, it directly fine-tunes on individual decompiled functions using the ground truth type and name information. It further uses data-flow analysis to propagate type information, data structure fields and leverages voting to resolve inconsistencies. \toolname goes beyond ReSym by proposing
two unique \textbf{\textit{training}} paradigms that more effectively train LLMs on the variable renaming problem. First, instead of simply teaching a model to generate names from a function body, \toolname teaches a model to consider the relation between names in the calling context and the names to analyze. We refer this paradigm as \textbf{{\em Context-aware Fine-tuning}}. Second, \toolname aligns the distribution of a model with the symbol preference of developers. We refer this technique as \textbf{{\em Symbol Preference Optimization (SymPO)}}. 

Although the program analysis components in both ReSym and \toolname are adapted from the standard data-flow analysis, they are different in both design and implementation. Specifically, 
the analysis in ReSym focuses on type inference and type checking, whereas the analysis in \toolname focuses on name propagation, which has a different nature. For example, given a simple copy operation, the left-hand-side and the right-hand-side variables must have the same types. However, the left-hand-side names are more general than those on the right.
That said, we agree with the reviewers that we may not have conceptual novelty regarding the combination of LLMs and program analysis. Therefore, we rewrote the contributions in the introduction section~(Section~\ref{sec:intro} of the paper), removing the corresponding claims. In addition, we only include a summary of our program analysis component in the main text~(Section~\ref{sec:method:infer} of the paper) and move the details to the Appendix~\ref{appdx:pa-and-voting}. We have also included the above discussion in the related work section.  




\subsubsection{\textbf{Clarify artifact availability}}
\label{sec:sub:art-aval}

We have submitted our artifact to the artifact evaluation track. Upon publication, we will publish our data, model checkpoints, and implementations. We clarify the artifact availability in Section~\ref{sec:setup}.

\subsubsection{\textbf{Clarify experimental setups}}
\label{sec:sub:exp-set}

We do not remove functions from test dataset. We clarify the point in Section~\ref{sec:method:sympo}, subsection ``Constructing the SymPO dataset''. We also revise the experimental setups~(Section~\ref{sec:setup}) according to new experiments introduced during the revision.

\subsubsection{\textbf{Comparison with ReSym}}
\label{sec:sub:cmp-resym}

We add ReSym as a baseline technique and compare \toolname with it. The results are in Table~\ref{tab:eval-performance}. \toolname demonstrates an improvement of 5.6 and 4.6 percentage points in terms of precision and recall on the DIRTY dataset; an improvement of 11.4 and 6.3 percentage points in terms of precision and recall on the VarCorpus dataset. Both experiments are in the most challenging split-by-binary setup. 
Moreover, \toolname demonstrates an improvement of 11.2 and 10.6 percentage points in terms of precision and recall in the split-by-function setup. It illustrates the effectiveness of \toolname over ReSym.

\subsubsection{\textbf{Comparison in the split-by-function setup}}
\label{sec:sub:cmp-split-by-func}

To fairly compare \toolname with the baseline techniques, we add experiments in the split-by-function setup. The results are discussed in Section~\ref{sec:sem-match}. \toolname outperforms the baseline techniques by 11.2 (ReSym) and 12.4 (VarBERT) percentage points in terms of precision; 10.6 (ReSym) and 13.6 (VarBERT) in terms of recall.

\subsubsection{\textbf{Experiments with more datasets}}
\label{sec:sub:more-ds}

We add experiments on datasets with different compiler optimization levels, from {\tt -O1} to {\tt -O3}. The results are discussed in Section~\ref{sec:eval-opt}. \toolname consistently outperforms both baseline techniques on all datasets.

\subsubsection{\textbf{Effects of model sizes}}
\label{sec:sub:study-model-size}

We add experiments in Section~\ref{sec:eval-size} to study the effectiveness of \toolname on different sizes of base models. The results show that the training paradigms of \toolname generalizes well to larger models. Especially, the 34B version of \toolname outperforms the 2B version by nearly 5 percentage points. That demonstrates the potential of \toolname on using LLMs in renaming variables.

\subsubsection{\textbf{Comparison with programming-focused black-box LLMs}}
\label{sec:sub:bb-clm}

We add CodeLlama-70B as a black-box LLM baseline. CodeLlama-70B is a large and programming-focused LLM. The results are shown in Table~\ref{tab:eval-blackbox-llm}. We can see that its performance is similar to GPT-3.5, and \toolname outperforms it by 15.3 and 12.8 percentage points in terms of precision and recall, respectively.


\subsubsection{\textbf{Generalization to rare names}}
\label{sec:sub:general-rare-name}

We discuss the generalization of \toolname to rare names in Section~\ref{sec:perf-general}. On top of the experiments of our previous submission, we further show that more than 95\% of rare names can be composed from frequently seen tokens. The details are in Fig.~\ref{fig:tok-freq}.


\subsubsection{ \textbf{Ablation study for the name validation algorithm}}
\label{sec:sub:abl-nv}

We discuss the effectiveness in Fig.~\ref{fig:eval-contrib} of the revised paper. The results show that the name validation algorithm contributes to the improvements by 5.4\%, yet its contribution is relatively less significant than the designs that help the model reason about contextual information (the training stage context-aware fine-tuning and inference stage context propagation contributes by 62.2\% and 18.9\%, respectively) and SymPO that teaches the model symbol preferences (which contributes by 13.5\%).


\subsubsection{ \textbf{Ablation study for the degree of context sensitivity}}
\label{sec:sub:abl-docs}

We discuss the effects of degree of context sensitivity in Appendix~\ref{appdx:ctx-sense}. The results show that with higher degree of context sensitivity, \toolname achieves better results. However, the improvements become marginal when the degree of context sensitivity is larger than 5.

\subsubsection{ \textbf{Semantics consistency and variable copies}}
\label{sec:sub:sem-copy}

We validate our assumption that names of two variables in the direct copy operations tend to be semantically consistent. The results are discussed in Appendix~\ref{appdx:assumption}. We study 920 pairs of variables from a well-known source code repository, and observe that the semantics of two variable names in direct copies are correlated for 78\% of the pairs, validating our assumption.


\subsubsection{ \textbf{Correlation between {\tt memset} and {\tt buffer}}}
\label{sec:sub:mem-buf}

We statistically test our observation that ``a variable is used as the first parameter to {\tt memset}'' is correlated with ``a model predict the name for this variable as {\tt buffer}''. The results are discussed in Appendix~\ref{appdx:corr}. The results conclude that there is statistically significant correlation between the aforementioned two events.

\subsubsection{ \textbf{Challenges in long-context code reasoning}}
\label{sec:sub:long-ctx-code}

We clarify in Appendix~\ref{appdx:long-ctx} that reasoning code in a long context remains a challenging task for even the advanced code models. The performance discrepancy can be 70\% (67.8 versus 20) for an advanced 70B code model across short-context coding tasks and long-context coding tasks. 



\subsection{Response to Revision Requirements}
\label{sec:rr}

\begin{myquote}
W1. Clarify the contribution compared to both LmPa and ReSym. This is especially important as the committee collectively felt the authors were not sufficiently transparent about this work given the availability of ReSym (and notification dates from other venues).
\end{myquote}

We clarify the unique contribution of \toolname over ReSym in Section~\ref{sec:sub:clarify-contrib}
of this document. On the other hand, LmPa is an arxiv paper and thus does not hinder the novelty of \toolname. 

\begin{myquote}
W2. Clarify the significance of this paper. For example, the program analysis component of this work appears to be reusing the ReSym technique on a different application -- this does not appear to be sufficiently compelling.
\end{myquote}

We clarify the significance of \toolname from two perspectives. 
\begin{itemize}
    \item Conceptually, as discussed in Section~\ref{sec:sub:clarify-contrib} of this document, \toolname proposes two unique training paradigms. It goes beyond a straight-forward fine-tuning of LLMs with post-processing~(i.e., the paradigm of ReSym).
    \item Empirically, as discussed in Sections~\ref{sec:sub:cmp-resym},~\ref{sec:sub:cmp-split-by-func},~\ref{sec:sub:more-ds} of this document, \toolname achieves improvements over ReSym that are of a comparable scale to that in existing work~\cite{dirty,varbert}. We clarify the comparison with baselines in Section~\ref{sec:sem-match} of the revised paper.
\end{itemize}
We have removed/toned-down our claim(s) regarding the program analysis component.

 
\begin{myquote}
W3. Clarify the availability of implementation and data. This is especially important given the earlier points concerning technical innovation.
\end{myquote}

Section~\ref{sec:sub:art-aval} clarifies that we submitted our artifacts to the AE track, and we will make them publicly available upon publication.

\begin{myquote}
W4. Clarify and justify the existing experimental settings (e.g., criteria for removing functions) and hypotheses (e.g., assuming variables copied always means semantic consistency).
\end{myquote}

We clarify in Section~\ref{sec:sub:exp-set} of this document that we do not remove functions from the test dataset. We use experiments, as discussed in Sections~\ref{sec:sub:sem-copy}~and~\ref{sec:sub:mem-buf} of this document, to support our assumptions and hypotheses.


\begin{myquote}
W5. Revise comparisons with previous work fairly. For example, the committee felt that claiming VarBERT's improvement of 4.5-5.1\% did not sufficiently reflect a fair basis for comparison (cf. 12.7\% improvement in Table 3 of VarBERT).
\end{myquote}

As discussed in Sections~\ref{sec:sub:cmp-resym}~and~\ref{sec:sub:cmp-split-by-func} of this document, we compare \toolname with previous work in both the split-by-binary setup and the split-by-function setup. In both setups, \toolname achieves improvements that are of a comparable scale with previous work~\cite{dirty,varbert}. 

We clarify the discussion in Section~\ref{sec:sem-match}, subsection ``Significance of improvements'' of our revised paper.

\begin{myquote}
E1. Consider additional datasets across multiple compiler optimization levels, and optionally, different architectures.
\end{myquote}

As discussed in Section~\ref{sec:sub:more-ds} of this document, we additionally run all techniques on the {\tt -O1}, {\tt -O2}, and {\tt -O3} version of the VarCorpus dataset. \toolname consistently outperforms the baseline techniques on all datasets. The improvement is more significant on binaries with less aggressive optimization because heavy optimizations make the decompiled code more different with source code, and thus harder to understand.

\begin{myquote}
E2. Augment the ablation study to investigate the impact of checking semantic consistency to alleviate hallucinations.
\end{myquote}

As discussed in Section~\ref{sec:sub:abl-nv}, we enhance our ablation study to show the effectiveness of each component. The results show that all components contribute to the improvements. Especially, the name validation algorithm~(i.e., the consistency checking algorithm) contributes by 5.4\%.



\begin{myquote}
E3. Clarify how composition of variable names from tokens can help generalize to rare or unseen names, with experiments to justify.
\end{myquote}

As discussed in Section~\ref{sec:sub:general-rare-name} of this document, we use experiments to show that 95\% of rare names can be composed from frequently seen tokens. The empirical results in Section~\ref{sec:perf-general} of the revised paper further show \toolname outperforms baselines on rare names.


\begin{myquote}
E4. Investigate the impact of more powerful base LLMs on GenNm. For example, add comparison with additional LLMs (e.g., CodeLlama 70B) to demonstrate efficacy over programming-focused LLMs, especially in settings with longer sequence lengths.
\end{myquote}

\begin{itemize}
    \item Due to the limited computing resources, we cannot afford fine-tuning a 70B model. Instead, we fine-tune CodeLlama-34B to demonstrate the effectiveness of \toolname on larger base models. As discussed in Section~\ref{sec:sub:study-model-size} of this document, \toolname is effective in training a larger code model on the renaming task, demonstrating better performance than the smaller models.
    \item As discussed in Section~\ref{sec:sub:bb-clm} of this document, we additionally use CodeLlama-70B as a black-box LLM and compare \toolname to it. The results are shown in Table~\ref{tab:eval-blackbox-llm} of our revised paper. The results show that \toolname outperforms the black-box larger programming-focused LLMs.
    \item  We analyze and discuss the challenges in reasoning long-context code in Section~\ref{sec:sub:long-ctx-code} of this document. Although advanced models support longer context, it remains an open challenge to conduct long-context coding tasks effectively.
\end{itemize}





\subsection{Response to Other Questions in Reviews}
\label{sec:other}

{
\centering
\subsection*{\textbf{Reviewer A}}
}


\begin{myquote}
RAQ1. marginal improvements in performance with respect to baselines.    
\end{myquote}

We clarify in Sections~\ref{sec:sub:cmp-resym}~and~\ref{sec:sub:cmp-split-by-func} of this document that our improvements are of comparable scale with previous work in this domain. 

\begin{myquote}
RAQ2. What impact does the $>$50\% variables having scores $\geq$4 have on the overall results of variable renaming?
\end{myquote}

We show in Fig.~\ref{fig:example-preds} concrete examples of variable names with different scores.

{
\centering
\subsection*{\textbf{Reviewer B}}
}

\begin{myquote}
RBQ1. Limited experimental evaluations with small models and few datasets.
\end{myquote}

\begin{itemize}
    \item As discussed in Sections~\ref{sec:sub:more-ds}~and~\ref{sec:sub:cmp-split-by-func} of this document, we run experiments on three additional datasets and one additional setup (the split-by-function setup).
    \item As discussed in Section~\ref{sec:sub:study-model-size} of this document, we additionally train \toolname on a larger code model~(CodeLlama-34B).
    \item We add CodeLlama-70B as a programming-focused black-box LLM baseline in Table~\ref{tab:eval-blackbox-llm} of the revised paper.
\end{itemize}


\begin{myquote}
RBQ2. Context Propagation: It is not clear how the context propagation algorithm adds the context to the generative model. Is the context simply appended to the query using special XML tags after the decompiled code and target variable names? A comprehensive example of all iterations during inference would help improve the understanding of the approach.
\end{myquote}

We revise Section~\ref{sec:method:ft-gen}, subsection ``Context Propagation'' to make the presentation clearer. Specifically, we add the intuition of context propagation at the beginning of the section, and revise the concrete example to make it easier to follow.


\begin{myquote}
RBQ3. Preferred names in SymPO dataset: The SymPO dataset uses variable names that are “significantly better” than the default prediction but not the ground truth. It is not clear what metric was used to identify better candidates. Was it through manual human inspection or other automated metrics? How is the best() function defined while creating the dataset?
\end{myquote}

We revise Section~\ref{sec:method:sympo} and explicitly state we use token-level precision and recall to find the ``best'' name. Also, we make it clearer how we filter out low-quality training functions.

\begin{myquote}
RBQ4. Black-box LLM benchmarks: GenNm outperforms GPT-3.5 and GPT-4. However, a more relevant comparison would be to larger code-generation LLMs like CodeLlama 70B. Intuitively, the results are expected as general-purpose GPT 3.5/4 models are not specially trained for programming tasks. Analyzing GenNM with CodeLlama-7B/CodeGemma-2B with larger variants of CodeLlama and CodeGemma would better highlight the efficacy of the proposed approach.
\end{myquote}

Please see RBQ1 for details.

\begin{myquote}
RBQ5. Ablation studies with longer sequence length: One of the motivations for the context propagation algorithm is that longer inputs are inefficient and may degrade performance. However, it would help to analyze this phenomenon in the code generation domain with a few concrete examples as modern code generation models like CodeLlama support sequence lengths in the order of tens of thousands of tokens.
\end{myquote}

As detailed in Section~\ref{sec:sub:long-ctx-code} of this document, we analyze and discuss the challenges of long-context coding tasks in the code generation domain. The performance of advanced long-context code language model (e.g., CodeLlama-70B) may degrade by 70\% across short-context and long-context coding tasks.

\begin{myquote}
RBQ4. Limited models and datasets: The experimental evaluation can be improved. Prior works like VarBert use at least three datasets and multiple optimization levels. It would be interesting to see the performance of GenNm on additional datasets like DIRE-dataset.
\end{myquote}

Please see RBQ1 for details. We include three more datasets with different optimizations, and one more dataset with different setup (i.e., the split-by-function setup). However, we do not include the DIRE dataset.
For one thing, the DIRE dataset only provides pre-processed data in textual format. \toolname needs to leverage the call graph information from the binary programs to propagate calling contexts. Moreover, the functions in the DIRE dataset are not stripped. The setup is not realistic in the reverse-engineering scenario.


\begin{myquote}
RBQ5. Detailed questions.
\begin{itemize}
    \item p6. It would be good to explain the intuition why the context would help improve the prediction precision.
    \item p7. "we remove the functions whose local information is not enough for the model to predict good names." Unclear how that was done.
    \item p9. The Assign-R rule looks strange. More justification is needed.
\end{itemize}
\end{myquote}

For the first two questions, please refer to RBQ2 and RBQ3 for details.

For the justification of the Assign-R rule, please see Section~\ref{sec:sub:sem-copy} of this document and Appendix~\ref{appdx:assumption} of the revised paper for details.




{
\centering
\subsection*{\textbf{Reviewer C}}
}

\begin{myquote}
RCQ1. I am not entire sure about the novelty of GenNm. GenNm "leverages the power of generative models," but it has been explored by LmPa [1] and ReSym [2]. What is the real novelty of GenNm over the existing work?
\end{myquote}

Please see W1 and W2 of the revision requirements~(Section~\ref{sec:rr} of this document).

\begin{myquote}
RCQ2. Specifically, the "symbol preference optimization" (SymPO) described in this paper is seemingly close to the similarity-based voting system in ReSym. Please compare them and showcase the novelty in SymPO.
\end{myquote}

SymPO is a training technique while similarity-based voting is a post-processing. We clarify the difference in Section~\ref{sec:sub:clarify-contrib} of this document.

\begin{myquote}
RCQ3. I find the claim of "alleviating the negative impacts of hallucination of the generative model" by checking the semantic consistency of predicted variable names rather strong (or, too strong to believe). Please evaluate how much this helps in your ablation study.
\end{myquote}

Please see E2 of the revision requirements for details.

\begin{myquote}
RCQ4. The claim "the generative model composes variable names from tokens, and thus can better generalize to rarely present or even unseen names" on Page 1 is both ungrounded and counter-intuitive. Please support your claim using citations or experiments.
\end{myquote}

Please see E3 of the revision requirements for details.


\begin{myquote}
RCQ5. Page 3. "Therefore, the model biases towards the name buffer after seeing the variable is used as the first argument to memset in the query." This is a pure guess without any evidence to prove. Please support your claim using experiments.
\end{myquote}

Please see Section~\ref{sec:sub:mem-buf} of this document for details.

\begin{myquote}
RCQ6. Is it possible that the performance gain of GenNm is because of the large amount of source code that the base LLMs have already been trained on, and as a result, many of these functions that LLMs have seen (and ingested) appear in the test set during evaluation?
\end{myquote}

We agree that the source code may already be in the pre-training data of an LLM as we have no way to prove or disprove. This is a question general for all LLM based techniques. On the other hand, we think it is a practical advantage of using LLMs as well because we benefit from the significant pre-training efforts.

That said, it is worth noting that decompiled code snippets are very different from source code snippets. For example, VarBERT shows that the editing distance between a decompiled function and its source code counterpart is over 300 characters on average~\cite{varbert}.

Moreover, our empirical observations with black-box LLMs (shown in Table~\ref{tab:eval-blackbox-llm} of the revised paper) demonstrates that there is still a significant gap between blackbox LLMs and GenNm, indicating the necessity of additional efforts of GenNm on leveraging LLMs' pre-training knowledge.



\begin{myquote}
RCQ7. Page 7. "We collect cases where GenNm\_ctx makes mistakes but has at least another response in the top 20 predictions that is significantly better." How is "significantly better" defined?

RCQ8. Page 8. "We remove functions with less than 5 statements and meanwhile do not have branches." Why are these functions removed? Do they still exist in the test set?
\end{myquote}

We revise Section~\ref{sec:method:sympo} and explicitly state we use token-level precision and recall to find the ``best'' name and we make it clearer how we filter out low-quality training functions. The revision emphasizes that we only remove functions in the training set, not the test set.


\begin{myquote}
RCQ9. Page 8. "If a variable is directly copied to another variable, ..., their names should be semantically consistent." Does this intuition hold in source code? Please evaluate it.
\end{myquote}

Please see Section~\ref{sec:sub:sem-copy} of this document and Section~\ref{appdx:assumption} of the revised paper for details.

\begin{myquote}
RCQ10. The evaluation is missing key comparisons against LmPa and ReSym.
\end{myquote}

Please see W2 of the revision requirements for details.


{
\centering
\subsection*{\textbf{Reviewer D}}
}


\begin{myquote}
RDQ1. Unfortunately, the paper does not provide any information details. Are the authors planning on providing the source code of their prototype?
\end{myquote}

Yes, we will provide the source code and data upon publication. We already submitted our implementations before the major revision to the artifacts evaluation track.

We clarify the artifact availability in the revised paper. Please see Section~\ref{sec:sub:art-aval} of this document for details.

\begin{myquote}
RDQ2. A detail that is not immediately clear from the current model description is how much of the calling context is used as part of the name generation: it seems that only the context of the 1st level caller is currently used, but I wonder how a larger context sensitivity would possibly improve the model (e.g., in cases where multiple "stub" functions may be called where each stub function has poor context, but the top level caller has rich semantics).
\end{myquote}

Please see Section~\ref{sec:sub:abl-docs} of this document for details.

